Towards Certifiable Adversarial Sample Detection

Convolutional Neural Networks (CNNs) are deployed in more and more classification systems, but adversarial samples can be maliciously crafted to trick them, and are becoming a real threat. There have been various proposals to improve CNNs' adversarial robustness but these all suffer performance penalties or other limitations. In this paper, we provide a new approach in the form of a certifiable adversarial detection scheme, the Certifiable Taboo Trap (CTT). The system can provide certifiable guarantees of detection of adversarial inputs for certain $l_{\infty}$ sizes on a reasonable assumption, namely that the training data have the same distribution as the test data. We develop and evaluate several versions of CTT with a range of defense capabilities, training overheads and certifiability on adversarial samples. Against adversaries with various $l_p$ norms, CTT outperforms existing defense methods that focus purely on improving network robustness. We show that CTT has small false positive rates on clean test data, minimal compute overheads when deployed, and can support complex security policies.

==> sections/acks.tex <==

\section*{Acknowledgements}
\textit{Partially supported with funds from Bosch-Forschungsstiftung
im Stifterverband.}

==> sections/discussion.tex <==
\section{Discussion}\label{sec:disc}

\subsection{Accuracy, Detection and Computation Overheads}

In this section we discuss the trade-offs facing the Sitatapatra user.
First and foremost,
the choice of keys has an impact on transferability.

% \begin{figure}[!h]
% \centering
% \begin{subfigure}{0.4\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/CW_lr_05_acc.png}
%   \caption{Change in Accuracies ($\Delta_{\mathsf{acc}}$).}
%   \label{fig:cwlr05_acc}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.4\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/CW_lr_05_detect.png}
%   \caption{Detection rates on the target model ($T_{\mathsf{det}}$)}
%   \label{fig:cwlr05_det}
% \end{subfigure}
% \caption{Changes in accuracies and detection rates of LeNet5 with various SDCM instrumentations}
% \label{fig:confusion}
% \end{figure}


In \Cref{fig:confusion}, we present a confusion matrix
with differently instrumented LeNet5 networks
attacking each other with C\&W attack for $20$ steps and a learning rate of $0.5$.
The chosen instrumentations are all second-order polynomials,
but with different coefficients.
It is apparent that Sitatapatra improves the accuracies
reported in \Cref{fig:cwlr05_acc}.
However, for the two polynomials, $2x^2+3x+5<6$ and $2x^2+4x+5<6$,
the behavior is different.
When using the adversarial samples from $2x^2+4x+5<6$ to attack $2x^2+3x+5<6$,
there is almost zero change in
accuracy between the source and the target model, but this relationship
does not hold in reverse.
The above phenomenon indicates that
the adversarial samples generated from one polynomial
are transferable to the other when the polynomials are too similar.
The same effect is observed in
the detector shown in \Cref{fig:cwlr05_det}: it is
easier to detect adversarial samples from $2x^2+4x+5<6$ to attack $2x^2+3x+5<6$.

This indicates that, when the models get
regularized to polynomials that are similar, the attacks between
them end up being transferable.
Fortunately, the detection rates remain relatively high even in this case.
Different polynomials restrict the activation value range in different ways.
In practice, we found that the smaller the range that
is available , \ie~the unpenalized space for
activations, the harder it is to train the network.
Intuitively, if the regularization applies too strict a constraint to
activation values,
the stochastic gradient descent process struggles to converge
in a space full of local minima.
However, a strong restriction on activation values caused detection
rates to improve. Thus, when deploying
models with Sitatapatra, the choice of polynomials affects base
accuracies, detection rates and training time.

Key choice brings efficiency considerations to
the table as well. Although training time for individual devices
may be a bearable cost in many applications, a substantial increase in
run-time computational cost will often be unacceptable.
%the instrumentation of a given CNN model
%means additional computational overheads
%and many devices can not afford it.
\Cref{tab:overhead} reflects
the total additional costs incurred
by using Sitatapatra in our evaluation models.
The \( < 7.5\% \) overhead we add
to the base network is small,
given that the models demonstrate
good defense and detection rates
against adversarial samples.
It is notable that during inference,
a detector module requires for each value
\( n \) fused multiply-add operations
to evaluate a \( n \)-degree \( f_k \) polynomial
using Horner's method~\citep{knuth1962evaluation},
and \( 1 \) additional operation for threshold comparison,
and thus utilize \( (n + 1) C_l H_l W_l \) operations
in total for the \( \ordinal{l} \) convolutional layer.
In our evaluation,
we set \( n = 2 \) by using second-order polynomials.
Additionally, a guard module
of the \( \ordinal{l} \) layer uses
channel-wise averaging, a fully connected layer,
a channel-wise scaling,
and element-wise multiplications for all activations,
which respectively require
\( C_l H_l W_l \), \( C_l^2 \), \( C_l \),
and \( C_l H_l W_l \) operations.

% \input{tables/overhead.tex}


\subsection{Key attribution}
While exploring which activations ended up triggering an
alarm with different Sitatapatra parameters, we
noticed that we could often attribute
the adversarial samples to the models used to
generate them.
In practice, this is a huge benefit, known as {\em traitor tracing} in
the crypto research community: if somebody notices an attack,
she can identify the compromised device and take appropriate action.
We conducted a simple experiment to evaluate how to identify
the source of a different adversarial sample.
We first produced models instrumented with different
polynomials using Sitatapatra and then generated the
adversarial examples.

In this simple experiment, we use
a support vector machine (SVM) to classify
the adversarial images based on the models generated them. The
SVM gets trained on the 5000 adversarial samples and gets
tested on a set of 10000 unseen adversarial images.
The training and test sets are disjoint.

\input{tables/overhead_and_attr.tex}

\Cref{tab:key_attribution} shows the
classification results for FGSM-generated samples and all
attacks combined.
Precision, Recall and F1 scores are reported.
In addition, we report the micro and macro aggregate
values of F1 scores -- micro counts the total true positive,
false negatives and false positives globally, whereas macro
takes label imbalance into account.

For both scenarios, we get a performance that is much better than random
guessing. First, it is easier to attribute
adversarial samples generated by the large coarse-grained
attacks. Second, for polynomials that are different enough,
the classification precision is high -- for just FGSM we get a
$90\%$ recognition rate, while with more attacks it falls to $81\%$
and $85\%$. For similar polynomials, we get worse performance, of around
$50\%$ for FGSM and around $30\%$ for all combined.
%Although better than random guesses, it still remains hard to
%tell the source of adversarialf samples if we have to consider all attacks.

This bring an additional trade-off -- training a lot of
different polynomials is hard, but it allows easier
identification of adversarial samples.
This then raises the question of scalability of the Sitatapatra model
instrumentation.

\subsection{Key size}

In 1883, the cryptographer Auguste Kerckhoffs enunciated a design principle that is used today: a system should withstand enemy capture, and in particular it should remain secure if everything about it, except the value of a key, becomes public knowledge~\citep{kerchoffs1883}.
Sitatapatra follows this principle -- as long as the key is secured, it will, at a minimal cost, provide an efficient way to protect against
low-cost attacks at scale. The only difference is that if an opponent
secures access to a system protected with Sitatapatra, then by observing
its inputs and outputs he can use standard optimisation methods to
construct adversarial samples. However these samples will no longer
transfer to a system with a different key.
One of the reasons why sample transferability is an
unsolved problem is because it has so far been hard to generate a wide
enough variety of models with enough difference between
them at scale.

Sitatapatra is the first attempt at this problem, and it shows
possibilities to embed different polynomial functions as keys to CNNs to block
transfer of adversarial samples.
Modern networks have hundreds of layers and channels, and thus can embed different keys at various parts improving key diversity.
% is possible to
% embed perhaps one key bit per channel per layer. Vision systems with
% hundreds of channels and dozens of layers will have enough key
% diversity to separate systems that are trained from scratch with
% entirely different keys. Whether this is a full solution to a given
% engineering problem will depend of whether the training
% overhead is acceptable. %Imagine trying to deploy a single model to a million devices. On such scale, even if it is just 20 epochs of additional training involved all-in-all it will be 20 million epochs.
The potential implication of having a key is important.
In the case where a camera vendor wants to sell the same vision system to
banks as in the mass market, it may be sufficient to have a completely
independent key for the cameras sold to each bank.
It will also be sensible for a mass-market vendor wants to
train its devices in perhaps several dozen different families, in order
to stop attacks scaling (a technique adopted by some makers of pay-TV
smartcards~\citep{And2008}). However it would not be practical to have an
individual key for each unit sold for a few dollars in a mass market.
The fact that adding keys to neural networks can improve its diversity
solves the problem of training multiple individual neural networks on the
same dataset, which is also known as a model ensemble.
In fact, our key instrumentation and the model identification from a model ensemble together can be seen as a stream of deployment, which also sufficiently increases the key space.
% We attempted to use a
% dynamically-rotated key in the hope that one would
% have to only train a single model and vary the key, but that resulted in
% extreme accuracy degradation.

% We therefore looked for a way to speed up model generation.
% We developed a different training methodology
% (compared to Algorithm 1 on page 5 in \citep{shumailov2018taboo}) and a
% different transfer function that is no longer dependent on
% activation distribution of a working model.

% We can train a model  to achieve high accuracy for a
% particular task given a small alarm rate, then start to iteratively
% increase the alarm rate but decrease the learning rate.
% We found that the models ended up converging near the original
% accuracy and produce the activation values inside the range of
% the transfer function.

% Second, we found we could fine-tune a new model based on an
% already instrumented one if the polynomials are not too different.
% We use Lagrange interpolation to generate unique polynomials with the
% same power as the training polynomial and that also pass through
% some nearby points. Polynomial similarity does however constrain the
% effective size of the key
% space, which means that attackers might find it easier to guess which
% polynomials a target system might use. It may also make adversarial
% sample attribution harder. The precise dynamics of key tweaking we
% leave to future work.


%\subsection{Attacking Sitatapatra}

%If attackers have full white-box access to the model, they can efficiently \emph{a)} deduce the polynomial used to bound theactivation spaces and \emph{b)} construct attacks that defeat detections.

%To demonstrate a worst-case attack, we changed the attack formulation used byTabacof~\etal~\citep{tabacof2016exploring} and included the TT regularization term into the generation of adversarial samples, which will then be optimized to stay inside the detection range so that no alarms are triggered.

%\begin{equation*}
%\centering
%	  \begin{aligned}
%\underset{D}{\text{minimize }}& ||D|| + C * H(p, p^A) + \alpha*d\\
%\text{subject to }& L \leq X + D \leq U	\\
%&p = f(X+D) \\
%&d = f_{\text{det}}(X+D)
%	  \end{aligned}
%\end{equation*}

%In the equation above, $p^A=[\mathbf{1}_{i=A}],$ is the adversarial probability target, $D$ is the perturbation, $C$ is the parameter to for the cross-entropy, $\alpha$ is a parameter for detection and $d$ represents the number of detected samples in the current batch.

%We ran the attacks against a TT instrumented LeNet5 network and observed the differences in the results produced with $\alpha=0$ and $\alpha=1$.

%\input{tables/penalty.tex}

%The results are shown in \Cref{tab:ataku}. Unsurprisingly, the percentage of detected samples decreased with an added term, but that resulted in an increased $l_2$ and decreased $l_\infty$ amplitude of the perturbations, calculated over 784 channels.
%This suggests the attacks are now specifically crafted to have more small perturbations in order to bypass detection.This difference is not universal and is directly connected to the model polynomial used  --- it works for that polynomial and for nearby ones, but not others.
%The attack network basically learned to manipulate features in a fine-grained fashion so as to keep the activations inside the detection boundaries. Nonetheless, 6--7\% of the adversarial samples still raised alarms.

% In practice, much more effective attacks against individual and aggregated Sitatapatra instrumented models could be constructed.
%Similarly, an additional penalizing term can be added to the attack's objective function either directly or through a smoother function to facilitate convergence.

%Despite this, Sitatapatra still provides protection and remains realistic.







==> tables/attribution.tex <==
\begin{table}[]
\begin{adjustbox}{scale=0.8,center}
\begin{tabular}{@{}l|lll|lll@{}}
\toprule
&\multicolumn{3}{c|}{FGSM}&\multicolumn{3}{c}{FGSM+DeepFool+C\&W}\\
Polynomial         & Precision & Recall & F1   & Precision & Recall & F1   \\\midrule
$0.1x^2-1x+2 < 3$  & \textbf{0.90}      & \textbf{0.90}   & 0.90 & 0.81      & 0.29   & 0.43 \\
$x^2-22x+120 < 10$ & \textbf{0.90}      & \textbf{0.89}   & 0.90 & \textbf{0.85}      & 0.28   & 0.42 \\
$2x^2+3x+5 < 6$    & 0.53      & 0.72   & 0.61 & 0.34      & 0.33   & 0.33 \\
$2x^2+4x+5 < 6$    & 0.56      & 0.35   & 0.43 & 0.30      & 0.69   & 0.41 \\ \midrule
Micro F1           & 0.72      & 0.72   & 0.72 & 0.40      & 0.40   & 0.40 \\
Macro F1           & \textbf{0.72}      & 0.72   & 0.71 & \textbf{0.57}      & 0.40   & 0.40 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Key attribution based on the adversarial sample produced.}
\label{tab:key_attribution}
\end{table}


==> tables/compare.tex <==
\begin{table}[!h]
\centering
\begin{adjustbox}{scale=0.8,center}
\begin{tabular}{@{}ll|l|ll|ll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{Pretrained}
& \multicolumn{2}{c}{Static Only}
& \multicolumn{2}{c}{Combined}       \\
&
&$\Delta_{\mathsf{Acc}}(\%)$
&$\Delta_{\mathsf{Acc}}(\%)$    &$T_{\mathsf{Det}}(\%)$
&$\Delta_{\mathsf{Acc}}(\%)$    &$T_{\mathsf{Det}}(\%)$
\\ \midrule
\multirow{3}{*}{FGSM}
 & $\epsilon=0.02$
 &0.70 &1.87  &0.00 &0.94 &0.00 \\
 & $\epsilon=0.08$
 &3.98 &15.78 &0.00 &9.14 &0.00 \\
 & $\epsilon=0.6$
 &3.05 &10.78 &0.19 &11.02 &22.28 \\
 \midrule
\multirow{2}{*}{DeepFool}
 & $i=50$
 &77.11 &78.20 &0.00 &87.42 &0.00 \\
 & $i=10$
 &9.22  &1.02  &0.00 &9.61 &0.00 \\
 \midrule
C\&W
 &$lr=0.5$
 &82.81 &91.02 &0.00 &89.61 &2.35 \\
 &$lr=1.0$
 &59.84 &90.39 &0.95 &78.91 &4.78 \\
 \midrule
$c=0.999$
 &$lr=0.5$
 &11.88 &57.50 &2.38 &25.31 &16.02 \\
 &$lr=1.0$
 &5.08  &45.00 &6.47 &12.66 &24.07 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of LeNet5 on MNIST with different instrumentations.
    $\Delta_{\mathsf{acc}}$ is the difference
    in accuracies and $T_{\mathsf{det}}$ is the detection rate.
    $l_2$ and $l_{\infty}$ are
    the averaged $l_2$ and $l_{\infty}$ norms of
    the distortions on all input images.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of steps and
    $lr$ is learning rate.
    $c$ is the confidence, the adversarial sample has to cause
    the misclassified class to have a probability above this given threshold.
    We use $20$ steps on C\&W.}
\label{tab:compare}
\end{table}

% &0.03515625 &0.1609375 &0.12578125 &- &- &5.11747989654541 &0.9028810620307922 &0.0515625 &0.0875 &0.0359375 &0.688584886106417 &0.931417603453999 &4.913985252380371 &0.9375062108039856 &0.04765625 &0.41484375 &0.3671875 &0.15508982651794906 &0.2848341580612277 &4.892731952667236 &0.9236176252365113\\
% &0.0046875 &0.05859375 &0.05390625 &- &- &5.780204486846924 &0.9455502033233643 &0.015625 &0.01875 &0.0031249999999999993 &0.8602972176238735 &0.967354598976778 &5.706935977935791 &0.9802315831184387 &0.00546875 &0.24609375 &0.240625 &0.2537238738999537 &0.37032561285154997 &5.494970989227295 &0.9740454196929932\\
% &0.00546875 &0.315625 &0.31015624999999997 &- &- &2.878287172317505 &0.6448896765708924 &0.2296875 &0.6765625 &0.44687499999999997 &0.004097492259764338 &0.11343711671285042 &1.0265390157699585 &0.24413472414016724 &0.01875 &0.9625 &0.94375 &0.0023873015873015872 &0.0 &1.569072151184082 &0.3500462770462036\\
% &0.85078125 &0.93984375 &0.08906249999999993 &- &- &1.7868361949920655 &0.4234331727027893 &0.98125 &0.98046875 &-0.0007812499999999556 &0.0 &0.2777777777777778 &0.8148597121238709 &0.20861342549324036 &0.9828125 &0.9796875 &-0.0031249999999999334 &0.0 &0.0 &1.1136931896209716 &0.2616474211215973\\



==> tables/detection_comp.tex <==
\begin{table}[!h]
\adjustbox{max width=\linewidth}{%
\centering
\begin{tabular}{@{}l|l|l|l|ll|l|@{}}
\toprule
Technique& $\theta$ & FGSM & DeepFool & New MACs & as \% & New Params \\ \midrule
% Taboo Trap & $f=1^{st}$ max percentile & 0.99 & 0.14 & 0 & 0 & 0\\ \midrule
% MagNet & & 1.0 & 1.0 & 137592 & 6 & 297 \\ \midrule
% \multirow{2}{*}{Metzen et al.}& 1 layer, DeepFool & 0.92  & 0.82  & $\sim 34810489$ & 1518 & 5945367 \\
% & 3 layers, DeepFool & 0.98  & 0.92  & $\sim 21767179$ & 949 & 4861597 \\
Taboo Trap & $P_{1}$ & 0.99 & 0.14 & \textbf{0} & \textbf{0} & \textbf{0}\\ \midrule
MagNet & & 1.0 & 1.0 & 190K & 20 & 297 \\ \midrule
\multirow{2}{*}{SafetyNet et al.}& 1 layer & 0.92  & 0.82  & 34.81M & 3622 & 5,95M \\
& 3 layers & 0.98  & 0.92  & 21.77M & 2265 & 4.86M \\
\bottomrule
\end{tabular}}
\caption{LeNet5 has 961K multiply-accumulate operations (MACs) and 17.75K parameters without defenses. SafetyNet is trained on the DeepFool adversarial samples. $P_{i}$ refers to the $i$th-percentile. FGSM $\epsilon=0.8$ is used. Overhead for MagNet is only calculated over the detector.}
\label{tab:len-act}
\end{table}


==> tables/dmcc.tex <==
\begin{table*}[]
\centering

\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|lllllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&         & \multicolumn{3}{c}{LeNet5}   & \multicolumn{3}{c}{MCifarNet} & \multicolumn{3}{c}{ResNet18-Cifar10}       \\
& Params  &Source   &Target   &$\Delta$  &Source   &Target   &$\Delta$   &Source  &Target  &$\Delta$ \\ \midrule
Clean
 &        &99.13    &99.09    &-         &89.04    &89.12    &-               &         &92.51    &- \\ \midrule
\multirow{3}{*}{FGSM}
 & $\epsilon=0.02$  &97.98    &92.05\\
 & $\epsilon=0.06$  &91.77    &98.13\\
 & $\epsilon=0.6$   &0.87     &2.89\\ \midrule
\multirow{2}{*}{DeepFool}
 & $i=50$           &12.40    &64.74\\
 & $i=100$          &13.96    &64.90\\ \midrule
\multirow{2}{*}{C\&W}
 &$i=100, lr=10^{-2}$   \\
 &$i=500, lr=5*10^{-3}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of adversarial samples with DMCC instrumentation.
    Source and Target are two models of the same topology but different DMCC
    instrumentations. $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of iterations for iterative methods like DeepFool
    and C\&W, $lr$ is learning rate.
    The LeNet5, MCifarNet and ResNet18-Cifar10 without defense have
    $99.03\%$, $87.56\%$ and $xx$ accuracies respectively. }
\label{tab:reg-effect}
\end{table*}


==> tables/l2_tab.tex <==
\begin{table*}[]
\centering

\begin{adjustbox}{scale=1.0,center}
%\begin{tabular}{@{}ll|llllll|llllll|llllll|llllll@{}}
% \begin{tabular}{@{}llllllllllllll@{}}
\begin{tabular}{@{}llllllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&
& \multicolumn{4}{c}{LeNet5}
& \multicolumn{4}{c}{MCifarNet} \\
% & \multicolumn{4}{c}{ResNet18-Cifar10} \\
%& \multicolumn{6}{c}{ResNet18-Cifar100} \\
&
& Acc     &Det     &$l_2$   &$l_{\infty}$
& Acc     &Det     &$l_2$   &$l_{\infty}$
% & Acc     &Det     &$l_2$   &$l_{\infty}$
%&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
\\ \midrule
Clean&
&99.13    &99.25   &-            &-
&89.51    &90.14   &-            &-
% &91.12    &93.58   &-            &-
%&75.91    &72.24    &-             &-       &-            &-
\\ \midrule
% \multicolumn{2}{c}{$l_{\infty}$ bounded attacks} &&
% \\
\multirow{5}{*}{FGM}
& $\epsilon=0.5$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=1.0$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=1.5$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=2.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=3.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{FGM w/ GE}
& $\epsilon=0.5$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=1.0$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=1.5$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=2.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=3.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{DeepFool}
& $\epsilon=0.5$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=1.0$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=1.5$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=2.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=3.0$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{Deepfool w/ GE}
& $\epsilon=0.02$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=0.05$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=0.1$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=0.2$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=0.3$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
$l_{2}$ Averaged&
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13


% \midrule
% \multirow{5}{*}{FGSM /w GE}
% & $\epsilon=0.02$
% &97.87 &99.15 &1.28 &0.00 &0.43 &0.02
% &28.41 &39.35 &10.94 &2.03 &0.97 &0.02
% &40.91 &60.94 &20.03 &1.68 &1.03 &0.02
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.05$
% &95.31 &98.44 &3.12 &0.00 &1.07 &0.05
% &25.28 &35.65 &10.37 &2.09 &2.38 &0.04
% &29.69 &44.32 &14.63 &0.25 &2.50 &0.05
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.1$
% &82.39 &96.31 &13.92 &0.00 &2.14 &0.10
% &18.04 &26.56 &8.52 &3.28 &4.47 &0.08
% &18.32 &29.40 &11.08 &17.63 &4.88 &0.09
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.15$
% &62.93 &92.61 &29.69 &0.00 &3.19 &0.15
% &11.22 &19.32 &8.10 &17.24 &6.54 &0.12
% &9.94 &23.44 &13.49 &93.85 &7.17 &0.13
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.35$
% &7.67 &32.10 &24.43 &0.00 &7.35 &0.35
% &1.42 &15.48 &14.06 &84.84 &14.21 &0.28
% &2.70 &14.63 &11.93 &91.86 &15.27 &0.30
% %&- &- &- &- &- &-
% \\
% \midrule
% \multirow{3}{*}{PGD}
% & $i=10$
% &64.63 &98.44 &33.81 &0.00 &1.57 &0.09
% &1.14 &41.90 &40.77 &1.84 &0.76 &0.02
% &12.12 &61.09 &48.97 &0.30 &0.82 &0.03
% %&0.08 &53.62 &53.54 &100.00 &0.50 &0.01
% \\
% & $i=20$
% &0.85 &98.44 &97.59 &0.00 &1.96 &0.12
% &0.28 &41.90 &41.62 &1.84 &0.76 &0.02
% &10.40 &61.09 &50.69 &0.30 &0.90 &0.04
% %&0.00 &53.62 &53.62 &100.00 &0.50 &0.01
% \\
% & $i=50$
% &0.00 &98.44 &98.44 &0.00 &1.96 &0.12
% &0.00 &41.90 &41.90 &1.84 &0.76 &0.02
% &7.43 &60.94 &53.51 &0.29 &1.03 &0.05
% %&0.00 &53.62 &53.62 &100.00 &0.50 &0.01
% \\
% \midrule
% \multirow{3}{*}{PGD /w GE}
% & $i=10$
% &65.06 &98.72 &33.66 &0.00 &1.61 &0.09
% &0.99 &43.61 &42.61 &1.89 &0.76 &0.02
% &13.21 &63.21 &50.00 &1.04 &0.83 &0.03
% %&- &- &- &- &- &-
% \\
% & $i=20$
% &0.85 &98.72 &97.87 &0.00 &1.99 &0.12
% &0.28 &43.61 &43.32 &1.89 &0.76 &0.02
% &11.22 &63.21 &51.99 &1.04 &0.92 &0.04
% %&- &- &- &- &- &-
% \\
% & $i=50$
% &0.00 &98.72 &98.72 &0.00 &2.00 &0.12
% &0.00 &43.61 &43.61 &1.89 &0.76 &0.02
% &8.24 &63.07 &54.83 &1.04 &1.06 &0.05
% %&- &- &- &- &- &-
% \\
% \midrule
% \multirow{2}{*}{DeepFool}
% & $i=50$
% &11.48 &98.91 &87.42 &0.00 &1.51 &0.39
% &0.23 &76.25 &76.02 &1.30 &0.38 &0.05
% &3.75 &77.27 &73.52 &7.63 &0.87 &0.10
% %&1.33 &71.33 &70.00 &0.00 &0.14 &0.02
% \\
% & $i=10$
% &89.61 &99.22 &9.61 &0.00 &1.44 &0.37
% &2.97 &76.17 &73.20 &1.30 &0.38 &0.05
% &6.33 &77.50 &71.17 &6.95 &0.81 &0.10
% %&2.58 &71.33 &68.75 &0.00 &0.13 &0.02
% \\
% \midrule
% \multirow{2}{*}{C\&W}
% &$lr=0.5$
% &4.38 &93.98 &89.61 &2.35 &2.95 &0.66
% &3.83 &11.48 &7.66 &67.41 &9.82 &0.25
% &2.73 &20.55 &17.81 &95.50 &10.11 &0.25
% %&0.39 &16.41 &16.02 &72.42 &6.78 &0.17
% \\
% &$lr=1.0$
% &1.56 &80.47 &78.91 &4.78 &3.74 &0.75
% &5.31 &13.91 &8.59 &92.02 &17.11 &0.43
% &3.52 &11.72 &8.20 &96.05 &17.84 &0.46
% %&0.62 &13.98 &13.36 &76.58 &12.28 &0.31
% \\
% \midrule
% % \multirow{2}{*}{C\&W $c=0.999$}
% C\&W
% &$lr=0.5$
% &4.61 &29.92 &25.31 &16.02 &5.22 &0.94
% &4.53 &4.77 &0.23 &99.10 &17.37 &0.61
% &3.05 &15.70 &12.66 &98.60 &12.63 &0.38
% %&1.56 &2.11 &0.55 &99.92 &15.56 &0.50
% \\
% $c=0.999$
% &$lr=1.0$
% &1.88 &14.53 &12.66 &24.07 &5.92 &0.98
% &7.19 &7.58 &0.39   &100.00 &23.58 &0.80
% &5.55 &8.67 &3.12 &98.72 &22.20 &0.72
% %&1.72 &0.78 &-0.94 &100.00 &21.76 &0.66
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    The performance of VTT with $l_{2}$ based attacks.
    The LeNet5, MCifarNet, ResNet18-Cifar10
    without instrumentations have
    $99.03\%$, $87.56\%$, and $xx$ accuracies respectively.
    Acc and Det represents the network's accuracy and VTT's detection ratio
    respectively.
    $l_{2}$ and $l_{\infty}$ are measured on the differences
    between generated adversarial samples and the original inputs.
    Notice, in this table, if an adversarial image is not found,
    we still return the perturbed image rather than the original input.
    }
    % The LeNet5, MCifarNet, ResNet18-Cifar10 and ResNet18-Cifar100
    % without instrumentations have
    % $99.03\%$, $87.56\%$, $xx$ and $xx$ accuracies respectively. }
\label{tab:combined}
\end{table*}


==> tables/lenet.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|lllll|lllllll|lllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
& \multicolumn{5}{c}{Pretrained}
& \multicolumn{7}{c}{Static Only}
& \multicolumn{7}{c}{Combined}       \\
& Params
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$l_2$ &$l_{\infty}$
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$S_{\mathsf{Det}}$  &$T_{\mathsf{Det}}$  &$l_2$ &$l_{\infty}$
&$S_{\mathsf{Acc}}$   &$T_{\mathsf{Acc}}$     &$\Delta$  &$S_{\mathsf{Det}}$  &$T_{\mathsf{Det}}$  &$l_2$ &$l_{\infty}$    \\ \midrule
Clean &
&99.02    &99.00    &-         &-    &-
&98.70    &98.75    &-         &-    &-    &-    &-
&99.13    &99.10    &-         &-    &-    &-    &-    \\ \midrule
\multirow{3}{*}{FGSM}
 & $\epsilon=0.02$
 &97.89 &98.98 &1.09 &0.42 &0.02 &96.95 &97.89 &0.94 &0.00 &13.33 &0.35 &0.02 &96.33 &98.20 &1.88 &0.00 &0.00 &0.41 &0.02\\
 & $\epsilon=0.08$
 &91.25 &95.94 &4.69 &1.65 &0.08 &74.69 &85.55 &10.86 &0.33 &11.30 &1.37 &0.08 &82.66 &97.03 &14.38 &0.00 &0.00 &1.64 &0.08\\
 & $\epsilon=0.6$
 &0.86 &4.14 &3.28 &11.90 &0.59 &2.34 &6.48 &4.14 &50.55 &68.50 &9.52 &0.58 &0.08 &7.89 &7.81 &21.81 &8.98 &11.84 &0.59\\
 \midrule
\multirow{2}{*}{DeepFool}
 & $i=10$
 &85.62 &96.72 &11.09 &1.75 &0.41 &98.36 &98.20 &-0.16 &0.00 &26.86 &0.81 &0.21 &98.28 &98.12 &-0.16 &0.00 &0.00 &1.11 &0.26\\
 & $i=50$
 &14.45 &92.19 &77.73 &1.85 &0.44 &32.11 &96.33 &64.22 &0.34 &14.19 &0.85 &0.21 &11.56 &98.05 &86.48 &0.18 &0.00 &1.16 &0.27\\
%  & $i=10, c=0.999$
%  &85.08 &93.98 &8.91 &1.79 &0.42 &98.12 &98.05 &-0.08 &0.00 &27.78 &0.81 &0.21 &98.28 &97.97 &-0.31 &0.00 &0.00 &1.11 &0.26\\
%  & $i=50, c=0.999$
%  &0.55 &31.56 &31.02 &2.88 &0.64 &22.97 &67.66 &44.69 &0.41 &11.34 &1.03 &0.24 &1.88 &96.25 &94.38 &0.24 &0.00 &1.57 &0.35\\
 \midrule
\multirow{2}{*}{C\&W}
 &$lr=0.5$
 &3.28 &86.88 &83.59 &3.10 &0.71 &4.61 &65.94 &61.33 &19.49 &50.78 &2.95 &0.69 &4.45 &93.05 &88.59 &2.95 &4.66 &2.91 &0.69\\
 &$lr=1.0$
 &0.39 &60.39 &60.00 &4.25 &0.76 &0.86 &36.41 &35.55 &39.57 &73.93 &3.90 &0.79 &0.31 &80.62 &80.31 &6.82 &10.38 &3.95 &0.77\\
 &$lr=0.5, c=0.999$
 &3.52 &16.09 &12.58 &5.12 &0.90 &5.16 &8.75 &3.59 &68.86 &93.14 &4.91 &0.94 &4.77 &41.48 &36.72 &15.51 &28.48 &4.89 &0.92\\
 &$lr=1.0, c=0.999$
 &0.47 &5.86 &5.39 &5.78 &0.95 &1.56 &1.88 &0.31 &86.03 &96.74 &5.71 &0.98 &0.55 &24.61 &24.06 &25.37 &37.03 &5.49 &0.97\\


\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of LeNet5 on MNIST with different instrumentations.
    Source generates adversarial samples and Target got attacked.
    S-Acc and T-Acc are the accuracies of the Source and Target
    with adversarial samples respectively, and $\Delta$ is the difference
    in accuracies.
    $l_2$ and $l_{\infty}$ are
    the averaged $l_2$ and $l_{\infty}$ norms of
    the distortions on input images.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of steps for DeepFool,
    $lr$ is learning rate for C\&W.
    $c$ is the confidence, the adversarial sample has to cause
    the misclassified class to have a probability above this threshold.
    We use $20$ steps on C\&W, and the polynomial parameters for
    source and target models are [2, 3, 5, 6] and [2, 4, 5, 6]
    respectively.
    }
\label{tab:lenet}
\end{table*}

% &0.03515625 &0.1609375 &0.12578125 &- &- &5.11747989654541 &0.9028810620307922 &0.0515625 &0.0875 &0.0359375 &0.688584886106417 &0.931417603453999 &4.913985252380371 &0.9375062108039856 &0.04765625 &0.41484375 &0.3671875 &0.15508982651794906 &0.2848341580612277 &4.892731952667236 &0.9236176252365113\\
% &0.0046875 &0.05859375 &0.05390625 &- &- &5.780204486846924 &0.9455502033233643 &0.015625 &0.01875 &0.0031249999999999993 &0.8602972176238735 &0.967354598976778 &5.706935977935791 &0.9802315831184387 &0.00546875 &0.24609375 &0.240625 &0.2537238738999537 &0.37032561285154997 &5.494970989227295 &0.9740454196929932\\
% &0.00546875 &0.315625 &0.31015624999999997 &- &- &2.878287172317505 &0.6448896765708924 &0.2296875 &0.6765625 &0.44687499999999997 &0.004097492259764338 &0.11343711671285042 &1.0265390157699585 &0.24413472414016724 &0.01875 &0.9625 &0.94375 &0.0023873015873015872 &0.0 &1.569072151184082 &0.3500462770462036\\
% &0.85078125 &0.93984375 &0.08906249999999993 &- &- &1.7868361949920655 &0.4234331727027893 &0.98125 &0.98046875 &-0.0007812499999999556 &0.0 &0.2777777777777778 &0.8148597121238709 &0.20861342549324036 &0.9828125 &0.9796875 &-0.0031249999999999334 &0.0 &0.0 &1.1136931896209716 &0.2616474211215973\\


==> tables/linf_tab.tex <==
\begin{table*}[]
\centering

\begin{adjustbox}{scale=1.0,center}
%\begin{tabular}{@{}ll|llllll|llllll|llllll|llllll@{}}
% \begin{tabular}{@{}llllllllllllll@{}}
\begin{tabular}{@{}llllllllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&
& \multicolumn{4}{c}{LeNet5}
& \multicolumn{4}{c}{MCifarNet} \\
% & \multicolumn{4}{c}{ResNet18-Cifar10} \\
%& \multicolumn{6}{c}{ResNet18-Cifar100} \\
&
& Acc     &Det     &$l_2$   &$l_{\infty}$
& Acc     &Det     &$l_2$   &$l_{\infty}$
% & Acc     &Det     &$l_2$   &$l_{\infty}$
%&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
\\ \midrule
Clean&
&99.13    &99.25   &-            &-
&89.51    &90.14   &-            &-
% &91.12    &93.58   &-            &-
%&75.91    &72.24    &-             &-       &-            &-
\\ \midrule
% \multicolumn{2}{c}{$l_{\infty}$ bounded attacks} &&
% \\
\multirow{5}{*}{FGSM}
& $\epsilon=0.02$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=0.05$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=0.1$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=0.2$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=0.3$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{FGSM GE}
& $\epsilon=0.02$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=0.05$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=0.1$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=0.2$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=0.3$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{BIM}
& $\epsilon=0.02$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=0.05$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=0.1$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=0.2$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=0.3$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
\multirow{5}{*}{BIM GE}
& $\epsilon=0.02$
&97.30 &98.44 &0.43 &0.02
&26.42 &38.64 &1.00 &0.02
% &39.29 &59.41 &1.03 &0.02
\\
& $\epsilon=0.05$
&5.26 &0.00 &1.07 &0.05
&10.09 &1.53 &2.43 &0.04
% &14.56 &0.75 &2.50 &0.05
\\
& $\epsilon=0.1$
&15.34 &0.00 &2.13 &0.10
&8.52 &3.17 &4.63 &0.09
% &11.13 &20.10 &4.84 &0.09
\\
& $\epsilon=0.2$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
& $\epsilon=0.3$
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13
\\
\midrule
$l_{\infty}$ Averaged&
&26.99 &0.00 &3.18 &0.15
&8.24 &18.11 &6.84 &0.13
% &12.50 &93.02 &7.12 &0.13


% \midrule
% \multirow{5}{*}{FGSM /w GE}
% & $\epsilon=0.02$
% &97.87 &99.15 &1.28 &0.00 &0.43 &0.02
% &28.41 &39.35 &10.94 &2.03 &0.97 &0.02
% &40.91 &60.94 &20.03 &1.68 &1.03 &0.02
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.05$
% &95.31 &98.44 &3.12 &0.00 &1.07 &0.05
% &25.28 &35.65 &10.37 &2.09 &2.38 &0.04
% &29.69 &44.32 &14.63 &0.25 &2.50 &0.05
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.1$
% &82.39 &96.31 &13.92 &0.00 &2.14 &0.10
% &18.04 &26.56 &8.52 &3.28 &4.47 &0.08
% &18.32 &29.40 &11.08 &17.63 &4.88 &0.09
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.15$
% &62.93 &92.61 &29.69 &0.00 &3.19 &0.15
% &11.22 &19.32 &8.10 &17.24 &6.54 &0.12
% &9.94 &23.44 &13.49 &93.85 &7.17 &0.13
% %&- &- &- &- &- &-
% \\
% & $\epsilon=0.35$
% &7.67 &32.10 &24.43 &0.00 &7.35 &0.35
% &1.42 &15.48 &14.06 &84.84 &14.21 &0.28
% &2.70 &14.63 &11.93 &91.86 &15.27 &0.30
% %&- &- &- &- &- &-
% \\
% \midrule
% \multirow{3}{*}{PGD}
% & $i=10$
% &64.63 &98.44 &33.81 &0.00 &1.57 &0.09
% &1.14 &41.90 &40.77 &1.84 &0.76 &0.02
% &12.12 &61.09 &48.97 &0.30 &0.82 &0.03
% %&0.08 &53.62 &53.54 &100.00 &0.50 &0.01
% \\
% & $i=20$
% &0.85 &98.44 &97.59 &0.00 &1.96 &0.12
% &0.28 &41.90 &41.62 &1.84 &0.76 &0.02
% &10.40 &61.09 &50.69 &0.30 &0.90 &0.04
% %&0.00 &53.62 &53.62 &100.00 &0.50 &0.01
% \\
% & $i=50$
% &0.00 &98.44 &98.44 &0.00 &1.96 &0.12
% &0.00 &41.90 &41.90 &1.84 &0.76 &0.02
% &7.43 &60.94 &53.51 &0.29 &1.03 &0.05
% %&0.00 &53.62 &53.62 &100.00 &0.50 &0.01
% \\
% \midrule
% \multirow{3}{*}{PGD /w GE}
% & $i=10$
% &65.06 &98.72 &33.66 &0.00 &1.61 &0.09
% &0.99 &43.61 &42.61 &1.89 &0.76 &0.02
% &13.21 &63.21 &50.00 &1.04 &0.83 &0.03
% %&- &- &- &- &- &-
% \\
% & $i=20$
% &0.85 &98.72 &97.87 &0.00 &1.99 &0.12
% &0.28 &43.61 &43.32 &1.89 &0.76 &0.02
% &11.22 &63.21 &51.99 &1.04 &0.92 &0.04
% %&- &- &- &- &- &-
% \\
% & $i=50$
% &0.00 &98.72 &98.72 &0.00 &2.00 &0.12
% &0.00 &43.61 &43.61 &1.89 &0.76 &0.02
% &8.24 &63.07 &54.83 &1.04 &1.06 &0.05
% %&- &- &- &- &- &-
% \\
% \midrule
% \multirow{2}{*}{DeepFool}
% & $i=50$
% &11.48 &98.91 &87.42 &0.00 &1.51 &0.39
% &0.23 &76.25 &76.02 &1.30 &0.38 &0.05
% &3.75 &77.27 &73.52 &7.63 &0.87 &0.10
% %&1.33 &71.33 &70.00 &0.00 &0.14 &0.02
% \\
% & $i=10$
% &89.61 &99.22 &9.61 &0.00 &1.44 &0.37
% &2.97 &76.17 &73.20 &1.30 &0.38 &0.05
% &6.33 &77.50 &71.17 &6.95 &0.81 &0.10
% %&2.58 &71.33 &68.75 &0.00 &0.13 &0.02
% \\
% \midrule
% \multirow{2}{*}{C\&W}
% &$lr=0.5$
% &4.38 &93.98 &89.61 &2.35 &2.95 &0.66
% &3.83 &11.48 &7.66 &67.41 &9.82 &0.25
% &2.73 &20.55 &17.81 &95.50 &10.11 &0.25
% %&0.39 &16.41 &16.02 &72.42 &6.78 &0.17
% \\
% &$lr=1.0$
% &1.56 &80.47 &78.91 &4.78 &3.74 &0.75
% &5.31 &13.91 &8.59 &92.02 &17.11 &0.43
% &3.52 &11.72 &8.20 &96.05 &17.84 &0.46
% %&0.62 &13.98 &13.36 &76.58 &12.28 &0.31
% \\
% \midrule
% % \multirow{2}{*}{C\&W $c=0.999$}
% C\&W
% &$lr=0.5$
% &4.61 &29.92 &25.31 &16.02 &5.22 &0.94
% &4.53 &4.77 &0.23 &99.10 &17.37 &0.61
% &3.05 &15.70 &12.66 &98.60 &12.63 &0.38
% %&1.56 &2.11 &0.55 &99.92 &15.56 &0.50
% \\
% $c=0.999$
% &$lr=1.0$
% &1.88 &14.53 &12.66 &24.07 &5.92 &0.98
% &7.19 &7.58 &0.39   &100.00 &23.58 &0.80
% &5.55 &8.67 &3.12 &98.72 &22.20 &0.72
% %&1.72 &0.78 &-0.94 &100.00 &21.76 &0.66
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    The performance of VTT with $l_{\infty}$ based attacks.
    The LeNet5, MCifarNet, ResNet18-Cifar10
    without instrumentations have
    $99.03\%$, $87.56\%$, and $xx$ accuracies respectively.
    Acc and Det represents the network's accuracy and VTT's detection ratio
    respectively.
    $l_{2}$ and $l_{\infty}$ are measured on the differences
    between generated adversarial samples and the original inputs.
    Notice, in this table, if an adversarial image is not found,
    we still return the perturbed image rather than the original input.
    }
\label{tab:combined}
\end{table*}


==> tables/overhead.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{scale=0.8}
\begin{tabular}{l|lllll}
    \toprule
    \multirow{2}{*}{Model}
        & \multicolumn{5}{c}{{\#FLOPs}} \\
    {}
        & original & detector & guard
        & total & overhead \\
    \midrule
    LeNet5
        & 480,500 & 28,160 & 7,660
        & 516,320 & 7.45\% \\
    ResNet18
        & 37,016,576 & 152,094 & 1,847,106
        & 39,015,776 & 5.40\% \\
    MCifarNet
        & 174,301,824 & 715,422 & 646,082
        & 175,663,328 & 0.64\% \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{%
    The computational costs,
    measured in the number of FLOPs,
    added by the detector and guard modules
    to the original network.
}\label{tab:overhead}
\end{table}


==> tables/overhead_and_attr.tex <==
\begin{figure}[!ht]
\begin{minipage}{0.48\textwidth}
\centering
\begin{adjustbox}{scale=0.6}
\begin{tabular}{l|lllll}
    \toprule
    \multirow{2}{*}{Model}
        & \multicolumn{5}{c}{{\#FLOPs}} \\
    {}
        & original & detector & guard
        & total & overhead \\
    \midrule
    LeNet5
        & 480,500 & 28,160 & 7,660
        & 516,320 & 7.45\% \\
    ResNet18
        & 37,016,576 & 152,094 & 1,847,106
        & 39,015,776 & 5.40\% \\
    MCifarNet
        & 174,301,824 & 715,422 & 646,082
        & 175,663,328 & 0.64\% \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{%
    The computational costs,
    measured in the number of FLOPs,
    added by the detector and guard modules
    to the original network.
}\label{tab:overhead}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\begin{adjustbox}{scale=0.6}
\begin{tabular}{@{}l|lll|lll@{}}
\toprule
&\multicolumn{3}{c|}{FGSM}&\multicolumn{3}{c}{FGSM+DeepFool+C\&W}\\
Polynomial         & Precision & Recall & F1   & Precision & Recall & F1   \\\midrule
$0.1x^2-1x+2 < 3$  & \textbf{0.90}      & \textbf{0.90}   & 0.90 & 0.81      & 0.29   & 0.43 \\
$x^2-22x+120 < 10$ & \textbf{0.90}      & \textbf{0.89}   & 0.90 & \textbf{0.85}      & 0.28   & 0.42 \\
$2x^2+3x+5 < 6$    & 0.53      & 0.72   & 0.61 & 0.34      & 0.33   & 0.33 \\
$2x^2+4x+5 < 6$    & 0.56      & 0.35   & 0.43 & 0.30      & 0.69   & 0.41 \\ \midrule
Micro F1           & 0.72      & 0.72   & 0.72 & 0.40      & 0.40   & 0.40 \\
Macro F1           & \textbf{0.72}      & 0.72   & 0.71 & \textbf{0.57}      & 0.40   & 0.40 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Key attribution based on the adversarial sample produced.}
\label{tab:key_attribution}
\end{minipage}
\end{figure}


==> tables/penalty.tex <==
\begin{table}

\begin{adjustbox}{width=0.4\linewidth,center}
\begin{tabular}{@{}l|lll@{}}
\toprule
           & $l_2$        & $l_{\infty}$    & Det (\%) \\ \midrule
$\alpha=1$ & \textbf{1.38} & 0.22 & 6 \\
$\alpha=0$ & 1.29 & \textbf{0.24} & 7 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{C-LBFGS generated perturbations with and without penalty for detection}
\label{tab:ataku}
\end{table}


==> tables/pretrain.tex <==
\begin{table*}[]
\centering

\begin{adjustbox}{width=\textwidth,center}
%\begin{tabular}{@{}ll|lllll|lllll|lllll|lllll@{}}
\begin{tabular}{@{}ll|lllll|lllll|lllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&
& \multicolumn{5}{c}{LeNet5}
& \multicolumn{5}{c}{MCifarNet}
& \multicolumn{5}{c}{ResNet18-Cifar10}
%& \multicolumn{5}{c}{ResNet18-Cifar100}   
\\
& Params
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$   &$l_2$   &$l_{\infty}$
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$   &$l_2$   &$l_{\infty}$
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$   &$l_2$   &$l_{\infty}$
%&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$   &$l_2$   &$l_{\infty}$
\\ \midrule
Clean&
&99.13    &99.25    &-             &-       &-
&89.51    &90.14    &-             &-       &-
&91.12    &93.58    &-             &-       &-
%&71.69    &72.04    &-             &-       &-
\\ \midrule
\multirow{3}{*}{FGSM}
& $\epsilon=0.02$
&98.20 &98.91 &0.70 &0.42 &0.02
&17.03 &24.22 &7.19 &0.98 &0.02
&18.05 &50.16 &32.11 &0.99 &0.02
%&12.97 &36.64 &23.67 &0.76 &0.01
\\
& $\epsilon=0.06$
&92.19 &96.17 &3.98 &1.65 &0.08
&2.89 &11.17 &8.28 &3.67 &0.07
&4.61 &22.66 &18.05 &3.71 &0.07
%&2.50 &15.08 &12.58 &2.92 &0.05
\\
& $\epsilon=0.6$
&0.55 &3.59 &3.05 &11.91 &0.59
&1.02 &7.81 &6.80 &20.98 &0.48
&0.00 &8.59 &8.59 &22.07 &0.50
%&0.16 &8.67 &8.52 &18.11 &0.42
\\
\midrule
\multirow{2}{*}{DeepFool}
& $i=50$
&14.92 &92.03 &77.11 &1.86 &0.44
&1.02 &27.34 &26.33 &0.20 &0.03
&1.02 &88.20 &87.19 &0.16 &0.02
%&1.95 &67.34 &65.39 &0.08 &0.01
\\
& $i=10$
&87.73 &96.95 &9.22 &1.76 &0.41
&1.80 &27.34 &25.55 &0.20 &0.03
&1.72 &88.20 &86.48 &0.16 &0.02
%&3.20 &67.34 &64.14 &0.08 &0.01
\\
\midrule
\multirow{2}{*}{C\&W}
&$lr=0.5$
&3.75 &86.56 &82.81 &3.09 &0.71
&2.03 &10.47 &8.44 &9.86 &0.24
&0.55 &15.00 &14.45 &10.02 &0.24
%&0.55 &10.47 &9.92 &7.14 &0.18
\\
&$lr=1.0$
&1.02 &60.86 &59.84 &4.25 &0.76
&5.00 &11.02 &6.02 &17.28 &0.44
&0.62 &12.81 &12.19 &17.75 &0.45
%&0.70 &9.22 &8.52 &12.88 &0.33
\\ \midrule
% \multirow{2}{*}{C\&W $c=0.999$}
C\&W
&$lr=0.5$
&3.91 &15.78 &11.88 &5.12 &0.90
&2.73 &4.69 &1.95 &15.89 &0.52
&1.09 &10.39 &9.30 &14.63 &0.43
%&0.86 &1.48 &0.62 &13.77 &0.42
\\
$c=0.999$
&$lr=1.0$
&1.09 &6.17 &5.08 &5.75 &0.95
&5.47 &5.23 &-0.23 &24.27 &0.77
&1.48 &8.83 &7.34 &25.35 &0.81
%&0.78 &1.41 &0.62 &19.89 &0.55
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of two pretrained models with different
    initializations on various datasets.
    Source and Target are two models of the same topology
    but different initialization point.
    $S_{\mathsf{Acc}}$ and $T_{\mathsf{Acc}}$ are the accuracies on
    source and target models.
    $l_2$ and $l_{\infty}$ are the norm values of the adversarial noise,
    larger norm values mean larger perturbations.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of iterations and $lr$ is the learning rate.
    $c$ is the confidence, the adversarial sample has to cause
    the misclassified class to have a probability above this given threshold.
    }
\label{tab:pretrain}
\end{table*}


==> tables/taboo.tex <==
\begin{table*}[!h]
\centering

\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{@{}ll|llllll|llllll@{}}
\toprule
% &         & \multicolumn{9}{c}{Networks} \\ \midrule
&
& \multicolumn{6}{c}{LeNet5}
& \multicolumn{6}{c}{MCifarNet}
\\
& Params
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
&$S_{\mathsf{Acc}}(\%)$     &$T_{\mathsf{Acc}}(\%)$    &$\Delta_{\mathsf{Acc}}(\%)$  &$T_{\mathsf{Det}}(\%)$ &$l_2$   &$l_{\infty}$
\\ \midrule
Clean&
&99.13    &99.25    &-             &-       &-            &-
&89.51    &90.14    &-             &-       &-            &-
\\ \midrule
\multirow{4}{*}{FGSM}
& $\epsilon=0.02$
&97.58 &99.45 &1.87 &0.00 &0.35 &0.02
&10.70 &21.41 &10.70 &1.41 &0.95 &0.02
\\
& $\epsilon=0.06$
&82.58 &98.36 &15.78 &0.00 &1.37 &0.08
&2.27 &11.17 &8.91 &10.47 &3.49 &0.06
\\
& $\epsilon=0.6$
&2.89 &13.67 &10.78 &0.19 &9.53 &0.58
&0.78 &9.22 &8.44 &78.63 &20.06 &0.46
\\
& mean
&- &- &9.48 &0.06 &- &-
&- &- &9.35 &30.17 &- &-
\\
\midrule
\multirow{3}{*}{DeepFool}
& $i=50$
&21.09 &99.30 &78.20 &0.00 &1.05 &0.25
&0.23 &69.53 &69.30 &2.49 &0.25 &0.03
\\
& $i=10$
&98.44 &99.45 &1.02 &0.00 &1.01 &0.25
&0.39 &69.53 &69.14 &2.49 &0.25 &0.03
\\
& mean
&- &- &39.61 &0.00 &- &-
&- &- &69.22 &2.49 &- &-
\\ \midrule
\multirow{3}{*}{C\&W}
&$lr=0.5$
&6.33 &97.34 &91.02 &0.00 &3.01 &0.70
&4.06 &11.33 &7.27 &89.25 &9.43 &0.24
\\
&$lr=1.0$
&1.41 &91.80 &90.39 &0.95 &3.99 &0.79
&9.45 &14.45 &5.00 &88.86 &16.33 &0.41
\\
& mean
&- &- &90.70 &0.48 &- &-
&- &- &6.14  &89.10 &- &-
\\
\midrule
% \multirow{2}{*}{C\&W $c=0.999$}
C\&W
&$lr=0.5$
&6.64 &64.14 &57.50 &2.38 &4.89 &0.92
&5.08 &3.59 &-1.48 &100.00 &17.95 &0.67
\\
$c=0.999$
&$lr=1.0$
&1.95 &46.95 &45.00 &6.47 &5.53 &0.97
&10.86 &7.50 &-3.36 &100.00 &22.87 &0.76
\\
& mean
&- &- &51.25 &4.43 &- &-
&- &- &-2.42  &100.00 &- &-
\\
\midrule
Mean
&
&- &- &43.50 &1.11 &- &-
&- &- &19.32 &52.62 &- &-
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Transferability of LeNet5 and MCifarNet
    with SCM (using Guard only).
    Source and Target are two models of the same topology but different
    SCM instrumentations.
    $\epsilon$ is a hyperparameter in FGSM,
    $i$ is the number of iterations and $lr$ is the learning rate.}
    % The LeNet5, MCifarNet, ResNet18-Cifar10 and ResNet18-Cifar100
    % without instrumentations have
    % $99.03\%$, $87.56\%$, $xx$ and $xx$ accuracies respectively. }
\label{tab:taboo}
\end{table*}

